Estimation of Constraint Admissible Invariant Set with Neural Lyapunov Function

Constraint admissible positively invariant (CAPI) sets play a pivotal role in ensuring safety in control and planning applications, such as the recursive feasibility guarantee of explicit reference governor and model predictive control. However, existing methods for finding CAPI sets for nonlinear systems are often limited to single equilibria or specific system dynamics. This limitation underscores the necessity for a method to construct a CAPI set for general reference tracking control and a broader range of systems. In this work, we leverage recent advancements in learning-based methods to derive Lyapunov functions, particularly focusing on those with piecewise-affine activation functions. Previous attempts to find an invariant set with the piecewise-affine neural Lyapunov function have focused on the estimation of the region of attraction with mixed integer programs. We propose a methodology to determine the maximal CAPI set for any reference with the neural Lyapunov function by transforming the problem into multiple linear programs. Additionally, to enhance applicability in real-time control scenarios, we introduce a learning-based approach to train the estimator, which infers the CAPI set from a given reference. The proposed approach is validated with multiple simulations to show that it can generate a valid CAPI set with the given neural Lyapunov functions for any reference. We also employ the proposed CAPI set estimation method in the explicit reference governor and demonstrate its effectiveness for constrained control.

==> note.tex <==

% \documentclass[letterpaper, 10 pt, conference]{ieeeconf}  % Comment this line out if you need a4paper

% %\documentclass[a4paper, 10pt, conference]{ieeeconf}      % Use this line for a4 paper

% \IEEEoverridecommandlockouts                              % This command is only needed if 
%                                                           % you want to use the \thanks command

% \overrideIEEEmargins                                      % Needed to meet printer requirements.
% \usepackage{graphics} % for pdf, bitmapped graphics files
% \usepackage{epsfig} % for postscript
% % \usepackage{xeCJK}
% %graphics files
% %\usepackage{mathptmx} % assumes new font selection scheme installed
% %\usepackage{times} % assumes new font selection scheme installed
% % \usepackage{caption}
% % \usepackage{subcaption}
% % \usepackage{subfigure}
% \usepackage{mathtools}
% \usepackage{amsmath} % assumes amsmath package installed
% \usepackage{amssymb}  % assumes amsmath package installe
% % \usepackage{algpseudocode}
% % \usepackage{algorithm}
% \usepackage[ruled, vlined, linesnumbered]{algorithm2e}
% % \usepackage{algorithmic}
% \usepackage{todonotes}
% \usepackage{xcolor}
% \usepackage{graphicx}
% \usepackage{caption,subcaption}
% \newcommand\colorcomment[1]{\textcolor{red}{#1}}
% \usepackage{multirow}
% \usepackage{mathrsfs}
% \usepackage{ctable} % for \specialrule command
% \usepackage{url}
% \usepackage{array,booktabs,ragged2e}
% \usepackage[english]{babel}
% \usepackage{gensymb}
% \usepackage{hhline}
% \usepackage{hyperref}
% \usepackage{amssymb} % for \longrightarrow
% \usepackage[T1]{fontenc} % for \symbol{92} 
% % \makeatletter
% % \algrenewcommand\ALG@beginalgorithmic{\footnotesize}
% % \makeatother
% \usepackage{amsmath}
% \usepackage{enumitem}
% %\usepackage{amsthm}
% %\theoremstyle{definition}
% % \usepackage{amsthm}
% % \usepackage{thmtools}
% \newtheorem{theorem}{Theorem}
% \newtheorem{problem}{Problem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{assumption}{Assumption}
% \newtheorem{proposition}{Proposition}
% \newtheorem{remark}{Remark}
% \newtheorem{definition}{Definition}
% % \declaretheorem[style=definition,numbered=yes]{definition}

% \renewcommand{\r}{{\mathbf r}}

% \newcommand{\z}{{\mathbf z}}
% \newcommand{\bmu}{{\bm{\mu}}}

% \newcommand{\A}{\mathcal{A}}
% \newcommand{\R}{\mathbb{R}}

% \newcommand{\U}{\mathcal{U}}
% \newcommand{\X}{\mathcal{X}}
% \newcommand{\Y}{{\mathbf Y}}
% \newcommand{\Z}{{\mathcal Z}}
% \newcommand{\cH}{{\mathcal H}}
% \newcommand{\x}{\mathbf{x}}
% \newcommand{\y}{\mathbf{y}}
% \renewcommand{\d}{\mathbf{d}}
% \renewcommand{\t}{\tau}
% \renewcommand{\v}{{\mathbf v}}
% \renewcommand{\u}{{\mathbf u}}
% \renewcommand{\o}{{\mathbf o}}
% \renewcommand{\a}{{\mathbf a}}
% \newcommand{\e}{{\mathbf e}}
% \newcommand{\s}{{\mathbf s}}
% \newcommand{\w}{{\mathbf w}}
% % \newcommand{\x}{{\mathbf x}}
% \newcommand{\m}{{\mathbf m}}
% \newcommand{\n}{{\mathbf n}}
% % \newcommand{\y}{{\mathbf y}}
% % \newcommand{\z}{{\mathbf z}}
% \newcommand{\g}{{\mathbf g}}
% \newcommand{\h}{{\mathbf h}}
% \newcommand{\p}{{\mathbf p}}
% \newcommand{\q}{{\mathbf q}}
% \newcommand{\T}{{\mathbf T}}
% \newcommand{\VV}{{\mathbf V}}
% \newcommand{\YY}{{\mathbf Y}}
% \newcommand{\ZZ}{{\mathbf Z}}
% \newcommand{\f}{{\mathbf f}}
% %\newcommand{\X}{{\mathcal{X}}
% %\newcommand{\U}{{\mathcal{U}}
% %\renewcommand{\O}{{\mathcal{O}}


% \newcommand{\expc}[1]{ {\{ #1 \} } }
% \newcommand{\expct}[1]{ {\{ #1 \}^T } }
% \newcommand{\expe}[1]{ {\otimes #1 } }
% \newcommand{\expet}[1]{ {{\otimes #1}^T} }

% \renewcommand{\O}{{\mathcal{O}}}
% \renewcommand{\L}{\mathcal{L}}
% \renewcommand{\S}{\mathcal{S}}
% % \renewcommand{\C}{\mathcal{C}}
% \newcommand{\uf}{{\overline{f}}}
% \newcommand{\lf}{\underline{f}}
% \newcommand{\RR}{\mathcal{R}}



% \title{\LARGE \bf
% Note - Invariant Set Computation}

% \author{Dabin Kim$^{1,2}$ and H. Jin Kim$^{1,2}$
% \thanks{1: Aerospace, 2:ASRI}
% \thanks{Dabin Kim and H. Jin Kim are with the Department of Aerospace Engineering, Seoul National University, Seoul 08826, South Korea (e-mail: dabin404@snu.ac.kr, hjinkim@snu.ac.kr).}
% }



% \begin{document}



% \maketitle
% \thispagestyle{empty}
% \pagestyle{empty}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{abstract}
% \end{abstract}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Introduction}

% Output admissible invariant set. 

% Compute invariant set based on solving LP on each cell of partition. 
% First, we develop our approach based on single-hidden layer ReLU network. Then, based on the fact that we can convert any deep relu network into single-hidden-layer ReLU network \cite{villani2023any}, we show how we can deal with controller and lyapunov function expressed with deep ReLU network.

% \section{Preliminary}

% \begin{align}
%     \theta_{3}=M_{1}\theta_{1} \oplus M_{2}\theta_{2}
% \end{align}
% \begin{align}
%     W_{3} &=
%     \begin{bmatrix}
%         M_{1}W_{1} & M_{2}W_{2}    
%     \end{bmatrix},
%     \hspace{2mm}
%     c_{3} = M_{1}c_{1} + M_{2}c_{2}, \\
%     H_{3} &= \begin{bmatrix}
%         H_{1} \\ H_{2}
%     \end{bmatrix}, \text{ and} \hspace{2mm}
%     b_{3} = \begin{bmatrix}
%         b_{1} \\ b_{2}
%     \end{bmatrix}
% \end{align}

% \section{Implementation of ReLU Lyapunov Function}
% Hyperplane arrangement, enumeration of cell

% \cite{rada2018new}

% PWA formulation of ReLU actived Neural network 
% \begin{align}
%     \text{NN}_{\text{ReLU}}(x,\theta) &= WD_{i}^{\theta}Hx + WD_{i}^{\theta}b+c \nonumber  \\
%     &\text{if } S_{i}^{\theta}Hx+S_{i}^{\theta}b \geq 0 
% \end{align}

% \section{Computation of Invariant Set}
% The unsafe set $\O$ is defined with set of inequalities $\O=\{(x,r)\in \R^{n} \times \R^{m} | c_{i}(x,r)\geq0\}$, its boundary $\partial \O$ is implicitly defined as $c(x)=0$. The set of admissible references is defined as $\RR=\{r\in\R^{m}| \overline{c}_{i}(r)\geq 0, i=1,...,n_{c}\}$. The reference dependent invariant set based on level set of Lyapunov function can be defined as
% \begin{align}
%     S(r) = \{x \in \R^{n} | V(x,r)\leq \Gamma(r), \Gamma(r)>0\}, \hspace{1mm} \forall r \in \RR.
% \end{align}
% The maximal safe level set of the Lyapunov function $\Gamma(r)$ can be found with 
% \begin{align}
%     \Gamma^{*}(r) = \min_{\mathcal{P}} \max_{\partial \O} V(x,r)
% \end{align}

% \section{Method}
% We need to identify which partition the given state is reside. One possible way is enuemrate all partitions from ReLU network \cite{} and compare the activation pattern of the state. However, this scales linearly to the number of partitions, which is inadequate since it exponentially increases as width and depth of the network increases. Another way is to use the structure of ReLU netowrk where each neuron makes hyperplane. 

% \section{Roadmap}
% \subsection{Steps}
% \begin{itemize}
%     \item Shallow network, develop invariant set based on derived Lyapunov function parameterized by ReLU activation NN.
%     \item Apply the invariant set into Explicit reference governor to compute DSM. 
%     \item 1) Co-optimize Lyapunov function and maximal invariant set, 2) Online computation of invariant set
% \end{itemize}

% \subsection{Possible Extensions}
% \begin{itemize}
%     \item How about deep network (which is equivalent to larger shallow network)?
%     \item Output-feedback control with NN perception
% \end{itemize}

% \section{Current Idea}
% \begin{enumerate}
%     \item From PWA dynamics and controller, find PWA Lyapunov function parameterized by NN with ReLU activation.
%     \item Following procedure from \cite{jouret2023safety}, build tree of polytope and corresponding hyperplanes (which will be used to find corresponding cell of arbitrary point)
%     \item From obstacle polytope, V-representation, vertices is acquired. Find which cell is active (possible violation occurs)
%     \item From active cells, get all vertices of cells, which are candidate points.
%     \item If affine transform (i.e. translation) is applied to the reference, apply same transformation to the candidate points. 
%     \item From the polytope tree, find corresponding cells where transformed candidate points reside. 
%     \item Classify each cell into Type 1 (where vertex of obstacle resides) and Type 2 (otherwise).
%     \item For Type 1 cell, we have to solve mixed-integer LP, and for Type 2, LP to get maximal Lyapunov value for in safe set. $\rightarrow$ Also for Type 1 cell, we can convert to LP with assumption that $\O$ is polytope by finding minimum of Lyapunov in obstacle region (obstacle region is now polytope). 
%     \item If we use PWQ Lyapunov function (as in \cite{chen2021learning}), opt problem becomes QP.
%     \item Complexity: Number of candidate cells $\#C$, $O(\#C \cdot \text{lp}())$. 
% \end{enumerate}

% \subsection{Tree of Partitions}
% For layer $l$, the hyperplane separating regions can be written recursively as 
% \begin{align}
%   \{ z^{(l-1)}\in \R^{n^{(l-1)}} | W_{n,*}^{l}z^{(l-1)}+b_{n}^{l}=m_{k} \}
% \end{align}
% % Since the output of layer $l-1$ can be reprsented as $z^{(l-1)}=\mathcal{E}$
% Since the partition is defined in input space, the hyperplane is expressed as
% \begin{align}
%   \mathcal{H}_{n,k}^{l}\{\RR_{j}\} = \{ x\in \R^{n} | W_{n}^{l}[\mathcal{E}_{j}^{(l-1)}x+\mathcal{G}_{j}^{(l-1)}]+b_{n}^{(l)} = m_{k}\}  
% \end{align}
% If a partition $\mathcal{R}_{j}$ is separated from the hyperplane $\mathcal{H}$, it generates two partitions from inequality. 

% The definition of the Chebyshev center,
% \begin{align}
%     \min_{\hat{x}, r} \Big\{ r:\|\hat{x}-x\|^{2}\leq r, \forall x \in Q \Big\}
% \end{align}
% Compute Chebyshev center for polytope $Q=\{x\in\R^{n}| Ax\leq b\}$
% \begin{align}
%     \max_{r, \hat{x}} \hspace{5mm} &r, \\
%     \text{s.t.} \hspace{3mm} &a_{i}\hat{x} + \|a_{i}\| r \leq b_{i}, \\
%     \text{and}\hspace{3mm} &r\geq 0
% \end{align}

% Seidel's LP (in C++ setting) is far superior in small dimension (2,3) and small number of constraints (I tried up to 7), than gurobi solver in Python (but core algorithm must be in C), which uses Simplex or barrier method. 

% \subsection{Applications}
% \begin{itemize}
%     \item Explicit Reference Governor
%     \item Motion Planning with Tree of Invariant Set \cite{brandt2023safe} \cite{danielson2016path}
% \end{itemize}

% \section{Note}
% % For bounded polytope obstacle, two polytopes are overlapping only if at least one of the vertex is inside the other polytope. \textcolor{red}{Maybe not.. I need to check.}

% \subsection{Idea about Partition Enumeration}
% \begin{itemize}
%     \item Tree of partition \cite{jouret2023safety}, activation pattern and neighboring polytope (RPM) \cite{vincent2021reachable}. 
%     \item Tree of partition can efficiently enumerate partitions which ReLU generates, but it might divide single partition (corresponds to single activation pattern) into multiple partitions. 
%     \item Reversly, RPM paper suggests how to get Polyhedron representation from activation pattern. But it does not give clue about which activation pattern actually gives legit partition (with finite volume). They propose marching method, which iteratively expand through region and find all partitions with realizable activation patterns. If we don't use marching method, we have to check $2^{N}$ number of all activation patterns, which is time consuming, where $N$ is the total number of neurons. 
%     \item We first generate the tree of partition, which gives us legit activation patterns. With set of each partition, if there are multiple partitions with same activation pattern, we replace the partition into one large overlapping partition, which is also convex polytope. Then, following \cite{vincent2021reachable}, we generate neighboring relation between partitions.
% \end{itemize}

% \section{Evaluation}
% Hybrid system, which cannot be done with SOS opt. 

% Example: Hierachical Control of F-16 aircraft \cite{heidlauf2018verification}.

% We can use Neural Lyapunov control method, which co-optimize control policy and lyapunov function. Or we can just verify the controller with finding lyapunov function. 
% In either way, we can use the proposed method to find  reference-dependent invariant set. 

% Other than many verification tool for learned controller exists \cite{jouret2023safety} where we can offline verification tool to check safety, when we use learned controller in dynamic environment, it is hard to show since it should be done online. We target to do this. 

% Ball-and-Plate system with explicit MPC. 4D. 
% Our approach may not scale well. For example,
% \begin{align}
%     \x(t+1)=I_{2} \otimes
%     \begin{bmatrix}
%         1 & 0.5 \\ 0 & 1
%     \end{bmatrix} \x(t) + I_{2} \otimes 
%     \begin{bmatrix}
%         0.125 \\ 0.5
%     \end{bmatrix} \u(t)
% \end{align}
% where $\x=[x,v_{x},y,v_{y}]^{T}$. 

% Cart-pole in Jang's paper. 4D case. 

% Single integrator navigation in dynamic scenario. 

% \textcolor{red}{Dubin's car cannot be stabilized by a continuous controller \cite{sontag1999stability}.}


% We can use \cite{wu2023neural} for finding lyapunov function for pre-defined controller, such as explicit MPC?

% Intersection of ROA, used for feedback motion planning. Invariant-set motion planning. 

% \section{Special Case}
% For special case, if ReLU network has zero bias terms, which was sufficient to derive lyapunov function for cart-pole of vertical quadrotor in \cite{wu2023neural}, it becomes special case for our algorithm. Note that in this case, the maximum number of partition is bounded to $2N$ where $N$ is the total number of neurons (\textcolor{red}{This is not true, but may be bounded to some smaller value}), regardless of the dimension of the system. 
% Also each parition shares single vertex, the origin. This simplifies our algorithm, and derive more efficient real-time computation. 

% However, in higher dimension and with many constraints, it is still infeasible to compute $\Gamma$ in real-time. In special cases, we can speed up its computation.
% First, if the Lyapunov function is convex, we can use convexity property, where any local optima is global optima. 
% If one partition has minimum gamma where its neighbor's solution are all larger than its, then we can conclude that such gamma is global solution. \textcolor{red}{need proof.}
% Second, for more special case, if the Lyapunov function is polyhedral function, we can compute the safe level set by formulating it in LP form, using its epigraph. (In such case, linear hybrid systems. linear system controlled with Explicit MPC.)
% \cite{kousoulidis2021polyhedral} \cite{berger2023counterexample}

% If we care about computation time, we can also use this method for invariant-set feedback motion planner \cite{danielson2016path}. Hybrid system, Pogobot. 

% \section{Theory}
% \begin{itemize}
%     \item Show that after pruning based on activation pattern, all partitions have non-empty intersection set with obstacle. 
% \end{itemize}

% Lyapunov function is piecewise-affine in general ReLU NN. 
% But in special case, if bias terms are all zero, it becomes polyhedral Lyapunov function.
% Polyhedral Lyapunov function can be learned for hybrid linear systems. by Berger et al. CDC 2022

% $\epsilon$-stability is discussed in Wu et al. Dai et al. enables small violation in Lyapunov condition, and it requires dynamics and controller should follow ReLU representation. 
% Chang et al., Zhou et al. can work on general nonlinear dynamics but only check Lyapunov condition for $\|x\|\geq \epsilon$. 

% \subsection{Verification}
% \begin{problem}[Optimization for Verification]    
% \begin{align}
%     \max_{\x \in \R^{n}} \hspace{3mm} &z = NN_{ReLU} (\x;\theta_{c}) \\
%     s.t. \hspace{4mm} &NN_{ReLU}(\x;\theta_{v})\leq \xi, \\
%     &\xi = NN_{ReLU}(\x;\theta_{E})
% \end{align}
% \end{problem}
% where $\xi$ is level set estimated from the estimator.
% If the problem has positive optimal value, it is counter-example. This optimization problem can be transformed to MILP problem which can found exact solution.

% Constraint function is parameterized by ReLU activated network. (Trainiable such as \cite{chou2020learning}) For special case, when the constraint is convex polytope, equivalently parameterized by single hidden layer NN. 

% \begin{align}
%     \max_{\x \in \R^{n}} \hspace{3mm} &A_{c} z - b_{c} \\
%     s.t. \hspace{4mm} &NN_{ReLU}(\x;\theta_{v})\leq \xi, \\
%     &\xi = NN_{ReLU}(\x;\theta_{E})
% \end{align}

% \subsection{Training}
% Loss function
% \begin{align}
%     \mathcal{L} = \sum_{i=1}^{N} \| NN_{ReLU}(\x_{i};\theta_{E}) - e_{i}^{*} \|
% \end{align}

% \section{References}
% \begin{itemize}
%     \item \cite{jouret2023safety} enumeration of partitions from deep neural networks of PWA activations.
%     \item 
% \end{itemize}


% \addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
%                                   % on the last page of the document manually. It shortens
%                                   % the textheight of the last page by a suitable amount.
%                                   % This command does not take effect until the next page
%                                   % so it should come on the page before the last. Make
%                                   % sure that you do not shorten the textheight too much.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \bibliographystyle{./bibtex/IEEEtran}
% \bibliography{./bibtex/IEEEabrv, ./bibtex/mybibfile} % from my IROS 2019 paper



% \end{document}

